Cross-modal Fundus Image Registration under Large FoV Disparity

Previous work on cross-modal fundus image registration (CMFIR) assumes small cross-modal Field-of-View (FoV) disparity. By contrast, this paper is targeted at a more challenging scenario with large FoV disparity, to which directly applying current methods fails. We propose Crop and Alignment for cross-modal fundus image Registration(CARe), a very simple yet effective method. Specifically, given an OCTA with smaller FoV as a source image and a wide-field color fundus photograph (wfCFP) as a target image, our Crop operation exploits the physiological structure of the retina to crop from the target image a sub-image with its FoV roughly aligned with that of the source. This operation allows us to re-purpose the previous small-FoV-disparity oriented methods for subsequent image registration. Moreover, we improve spatial transformation by a double-fitting based Alignment module that utilizes the classical RANSAC algorithm and polynomial-based coordinate fitting in a sequential manner. Extensive experiments on a newly developed test set of 60 OCTA-wfCFP pairs verify the viability of CARe for CMFIR.

==> tables/tab_order.tex <==
% \begin{table}[!htb]
% \centering
% \renewcommand{\arraystretch}{1.1}
% \caption{\textbf{Results under different degree of polynomial fitting}. 
% }\label{tab:order}
% \scalebox{1.25}{
% \begin{tabular}{@{}l|c|c|c|c|c@{}}
% \toprule
% \textbf{Degree} & 1 & 2 & 3 & 4 & 5 \\
% \hline
% \makecell[c]{AUC $[\%]\uparrow$} & 88.8 & \textbf{89.6} & 87.1 & 82.2 & 77.6\\
% \bottomrule
% \end{tabular}
% }
% \end{table}

\begin{figure}[!tb] %插入图片
\centering %图片居中

\begin{tikzpicture} %tikz图片

\begin{axis}[
    xlabel=degree, %横坐标名
    ylabel=AUC, %纵坐标名
    tick align=outside, %刻度在外显式
    legend style={at={(0.5,-0.2)},anchor=north} %图例在图下方显示
    ]

%第一条线，mark是折线标示形状
\addplot[sharp plot,mark=*,blue] plot coordinates { 
    (1,88.8)
    (2,89.6)
    (3,87.1)
    (4,82.2)
    (5,77.6)
};

%图例里名字
%\addlegendentry{case 1}

\end{axis}
\end{tikzpicture}
\caption{Results under different degree of polynomial fitting}
\label{fig:degree}
\end{figure}
